Dealing with Missing Modalities in Multimodal Recommendation: a Feature Propagation-based Approach

Multimodal recommender systems work by augmenting the representation of the products in the catalogue through multimodal features extracted from images, textual descriptions, or audio tracks characterising such products. Nevertheless, in real-world applications, only a limited percentage of products come with multimodal content to extract meaningful features from, making it hard to provide accurate recommendations. To the best of our knowledge, very few attention has been put into the problem of missing modalities in multimodal recommendation so far. To this end, our paper comes as a preliminary attempt to formalise and address such an issue. Inspired by the recent advances in graph representation learning, we propose to re-sketch the missing modalities problem as a problem of missing graph node features to apply the state-of-the-art feature propagation algorithm eventually. Technically, we first project the user-item graph into an item-item one based on co-interactions. Then, leveraging the multimodal similarities among co-interacted items, we apply a modified version of the feature propagation technique to impute the missing multimodal features. Adopted as a pre-processing stage for two recent multimodal recommender systems, our simple approach performs better than other shallower solutions on three popular datasets.

==> src/limitations_future.tex <==
\section{Limitations and future directions}
\label{sec:limitations}
Despite the competitive performance results of FeatProp, we believe the proposed framework and methodology may still have room for improvement. Indeed, we acknowledge some unexpected trends in the FeatProp performance, especially when considering specific missing modalities settings. Moreover, the observed results raised more general doubts regarding the injection of multimodal features into any multimodal recommender system. Under this light, this section begins with pointing out such limitations. Later, it discusses possible directions for future enhancements of the FeatProp framework and multimodal recommendation in general.

\subsection{Performance and conceptual limitations}
The recognised limitations mainly fall into two categories: (i) \textbf{performance} limitations of our proposed approach in specific missing modalities settings; (ii) \textbf{conceptual} limitations, intended as how multimodal features are generally injected in any multimodal recommender system. We present them in the following.

\subsubsection{FeatProp with high missing modalities rates} In the original FeatProp paper~\cite{DBLP:conf/log/RossiK0C0B22}, the authors observe that the proposed algorithm is generally capable of tackling the issue of missing node features even with increasing missing features percentages. In fact, while performance generally tends to decrease with higher missing percentages for most of the other compared baselines, the introduced technique provides quite stable behaviours and the performance distance to the baselines widens. 

Conversely, with our FeatProp solution, we notice the method largely outperforms the other solutions, but following a decreasing trend with higher missing modalities percentages (at 80\% or 90\% it might get even lower than the other approaches). We deem it is worth investigating the trend, possibly exploring other multimodal recommendation models and/or datasets (to confirm the results) or trying wider sets of hyper-parameter values for the FeatProp algorithm (e.g., top-$n$ sparsifications and propagation layers).  

\subsubsection{The unreasonable behaviour of low-quality modalities} As already discussed in the results section, we observe an unexpected trend regarding the Zeros baseline, whose imputed missing multimodal features may be defined, for obvious reasons, as ``low-quality'' ones. Indeed, we notice its overall incredibly-high performance at 80\% or 90\% of missing modalities. In fact, on the \texttt{FREEDOM} recommendation model, we see the performance is even increasing along with the percentage of missing modalities.

We believe these outcomes may unintentionally have risen an important research question: as ``low-quality'' multimodal features injected into multimodal recommender systems are providing improved recommendation performance to ``higher-quality'' multimodal features (e.g., those imputed by FeatProp), \textbf{are we really leveraging multimodality in recommendation the right way?} We hope these side results from the current work might represent a possible starting point towards the next generation of multimodal recommender systems. 

\subsection{New perspectives in FeatProp and multimodal recommendation}
\label{sec:new_perspectives}
Motivated by the outlined limitations, in the following, we propose possible future directions regarding the FeatProp algorithm and multimodal recommendation in general.  

\subsubsection{Additional missing modalities scenarios} 
% For the sake of this work, we limited our focus to missing modalities settings where we assume the percentage of missing features is the same across all modalities. However, the scenario may be further explored by considering other dimensions. In this respect, it would be interesting to assess the performance of FeatProp with different percentages of missing features for each modality (e.g., 30\% of items do not have the \textbf{visual} modality, 20\% of items do not have the \textbf{textual} modality, and 50\% of the items do not have \textbf{both} modalities). Indeed, such a setting would provide a wider range of real-world scenarios to actually test the soundness and effectiveness of the proposed approach. Moreover, it should be pointed out that selecting items with one (or more) missing modalities at \textbf{random} may not be the most proper strategy to replicate a \textbf{real-world} scenario in the e-commerce domain. The lack of multimodal content describing items is not necessarily a random phenomenon, but it might follow a more precise pattern and schema (e.g., the images of all the products advertised by one company may not be available due to technical issues in the company's infrastructure). Additionally, the missing modalities trend could also vary over time, posing a new bunch of interesting challenges to be addressed. We intend to work towards all the outlined directions, possibly replacing the random sampling of missing modalities items. For instance, a simple (but more realistic) solution would be to build the initial recommendation dataset by retrieving all items in the catalogue, independently on the availability of their multimodal content; in this way, the missing modalities percentage would be defined by real-world trends, and experiments could be repeated over time to test the robustness of our approach. Ideally, we plan to create online dataset repositories in the e-commerce (and similar) domains whose multimodal content is collected at different timestamps.

In this work, we focused on missing modalities by assuming uniformity in the percentage of missing features across all modalities. However, exploring this scenario further, we propose evaluating FeatProp's performance with varying percentages of missing features for each modality. 

For example, assessing scenarios where 30\% of items lack visual modality, 20\% textual modality, and 50\% both would offer a broader understanding of real-world applicability. Furthermore, it is crucial to acknowledge that randomly selecting items with missing modalities may not accurately represent real-world scenarios in e-commerce. The absence of multimodal content could follow specific patterns, such as technical issues in a company's infrastructure, and this trend may vary over time, introducing new challenges.

We plan to refine our approach by replacing random sampling with a more realistic strategy. For instance, building the initial recommendation dataset regardless of multimodal content availability would mirror real-world trends, enabling experiments to be conducted over time for robustness testing. Ultimately, we aim to establish online dataset repositories in e-commerce (and similar domains) storing multimodal data with varying modalities availability rates at different timestamps.

\subsubsection{Reconstructing one modality through other modalities} Assuming each modality comes with different percentages of missing features (see the previous section), an extreme scenario is to entirely reconstruct one modality through the other ones. 

For instance, let us consider the toy example where the ego item is missing the \textbf{visual} modality; moreover, the same item is connected, in its neighborhood, to other items whose available modalities are only \textbf{textual} and/or \textbf{audio}. By applying the FeatProp algorithm as proposed in this work, the missing \textbf{visual} features of the ego item would not receive any \textbf{visual} contribution from the close neighbors, completely failing in the feature imputation. 

This ``blind spot'' in our solution may be addressed by re-thinking the FeatProp algorithm in such a way the features of different modalities can interact one another. Indeed, the idea would be to leverage the concept of intra- and inter-item \textbf{modalities alignment}, intended as the degree of ``semantic'' modalities similarity on the same item and on items directly-connected in the item-item graph, respectively. For this reason, we deem the importance to exploit multimodal features extracted through multimodal-by-design deep learning models (such as CLIP~\cite{DBLP:conf/icml/RadfordKHRGASAM21}) that are specifically trained to project the features of different modalities to the same ``semantic'' space; in fact, this appears to be a recent trend in the literature~\cite{DBLP:journals/corr/abs-2310-20343}.

\subsubsection{Using modalities on user-item interactions} Building the item-item graph (necessary to run the FeatProp algorithm) involves the projection of the user-item graph to the item-item one. However, this projection is not bind to leverage \textbf{only items co-interactions}. In domains such as e-commerce, the recorded user-item interactions may convey other rich sources of information that are not generally exploited in the realm of multimodal recommendation, for instance \textbf{textual reviews}~\cite{DBLP:conf/emnlp/WuWQGHX19, DBLP:conf/www/0012OM21, DBLP:conf/sigir/ShuaiZWSHWL22}. 

On popular selling platforms (e.g., Amazon) users generally express their opinion about products and services to share their experience with other interested users, thus creating a collaborative network of comments and ideas. This content may be suitably used to enrich the information underlying each user-item interaction in the system, whose nature is not always easy to disentangle (considering an implicit feedback scenario). Driving from the textual features extracted from reviews, we may propose a slightly different version of the Assumption in~\Cref{sec:feat_prop_for_mm_recsys}, namely:
\begin{assumption_rev}
    In a multimodal recommendation scenario, where users' reviews are also available, it is safe to assume that co-interacted items (i.e., items being interacted by the same users) which were reviewed in a similar manner may be characterised by similar multimodal content.
\end{assumption_rev}
Intuitively, this means two items are similar if the users who have reviewed them have expressed (on average) the same comments and opinions. Note that the so-calculated item-item similarity graph would derive from the \textbf{textual} modality that, differently from the usual cases, here accounts for \textbf{the user-item interactions rather than the single users or items}. 

This intuition opens to imputing the missing modalities \textbf{on items} through the available modalities \textbf{on the user-item interactions}. To the best of our knowledge, this represents something completely unexplored in the current literature, as we are not only proposing to reconstruct one modality through other ones, but also on different sources (i.e., items \textit{vs.} user-item interactions).

\subsubsection{The quality of multimodal features} We believe that answering the question \textbf{are we really leveraging multimodality in recommendation the right way?} must necessary involve assessing the \textbf{quality} of the multimodal features injected in the multimodal recommendation system. However, the exact meaning of \textbf{quality} in this context is truly disputable. 

For instance, let us consider the photograph of a pair of red shoes, and let us extract its visual features through a pre-trained ResNet50, whose ultimate purpose is to classify the input image. Indeed, we may assume the \textbf{quality} of the extracted visual feature is determined by the \textbf{alignment degree} between the original image content and how the pre-trained ResNet50 has classified that content. This means that if the ResNet50 has classified the image as ``pair of shoes'' it is safe to state the extracted visual features will be high-quality, while they will be low-quality otherwise. 

Intuitively, high-quality multimodal features should eventually lead to improved recommendation performance. Nevertheless, the empirical evidence from the presented results suggests that also low-level-by-design features (e.g., vectors with all zero values) can still provide improved recommendation performance. Thus, the open research question becomes: \textbf{is multimodal recommendation able to recognise the quality of multimodal features?}
